Non-adversarial training of Neural SDEs with signature kernel scores

Neural SDEs are continuous-time generative models for sequential data. State-of-the-art performance for irregular time series generation has been previously obtained by training these models adversarially as GANs. However, as typical for GAN architectures, training is notoriously unstable, often suffers from mode collapse, and requires specialised techniques such as weight clipping and gradient penalty to mitigate these issues. In this paper, we introduce a novel class of scoring rules on pathspace based on signature kernels and use them as objective for training Neural SDEs non-adversarially. By showing strict properness of such kernel scores and consistency of the corresponding estimators, we provide existence and uniqueness guarantees for the minimiser. With this formulation, evaluating the generator-discriminator pair amounts to solving a system of linear path-dependent PDEs which allows for memory-efficient adjoint-based backpropagation. Moreover, because the proposed kernel scores are well-defined for paths with values in infinite dimensional spaces of functions, our framework can be easily extended to generate spatiotemporal data. Our procedure permits conditioning on a rich variety of market conditions and significantly outperforms alternative ways of training Neural SDEs on a variety of tasks including the simulation of rough volatility models, the conditional probabilistic forecasts of real-world forex pairs where the conditioning variable is an observed past trajectory, and the mesh-free generation of limit order book dynamics.

==> header.tex <==
\usepackage{eurosym}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{color}
\usepackage[dvipsnames]{xcolor}
\usepackage{subcaption,siunitx,booktabs}
\usepackage{mathrsfs}
% \usepackage[author={Oana}]{pdfcomment}
% \usepackage[color=yellow]{todonotes}
\usepackage{titling}
\usepackage{lipsum}
\usepackage{soul}
\usepackage{bm}
\usepackage{bbm}
\usepackage{comment}
\usepackage{enumerate}
\usepackage{framed}
% \usepackage[top=1in, bottom=1.25in, left=1.10in, right=1.10in]{geometry}
\usepackage{appendix}
\usepackage{stmaryrd} 
\usepackage{xcolor}
\usepackage{cleveref}
\usepackage{shuffle}
\usepackage{parskip}
\usepackage{url}
\usepackage{mathtools}
\usepackage{tikz-cd}
% \usepackage[noend]{algpseudocode}
\usepackage{algorithm}
\usepackage{booktabs}
\usepackage{algorithmic}
% \usepackage{subfigure}
\usepackage{subcaption}


\let\Algorithm\algorithm
% \renewcommand\algorithm[1][]{\Algorithm[#1]\setstretch{1.4}}

\setcounter{MaxMatrixCols}{10}

%TCIDATA{OutputFilter=Latex.dll}
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{<META NAME="SaveForMode" CONTENT="1">}
%TCIDATA{BibliographyScheme=Manual}
%TCIDATA{LastRevised=Monday, January 25, 2021 10:59:08}
%TCIDATA{<META NAME="GraphicsSave" CONTENT="32">}

\textwidth 17cm \textheight 23cm
\topmargin -1.5cm \oddsidemargin -0.5cm \evensidemargin -0.5cm 
\newtheorem{theorem}{Theorem}
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
% \newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{solution}[theorem]{Solution}
%\newtheorem{proof}[theorem]{Proof}
\newtheorem{summary}[theorem]{Summary}
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\providecommand\bv{\boldsymbol{v}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\oov}{\overline{\overline{v}}}
\newcommand{\ooh}{\overline{\overline{h}}}
\newcommand{\oW}{\overline{W}}
\newcommand{\restr}[1]{|_{#1}}
%\newcommand{\dd}{\,\mathrm{d}}
\renewcommand{\thefootnote}{\arabic{footnote}}
\def\DIV{{\bm \nabla \cdot}}
\def\CURL{{\bm {\nabla \times}}}
\newcommand{\reallywidehat}{\widehat}
\newcommand{\dy}{\, \mathrm{d}\mathbf{y}}
\newcommand{\dd}{\,\mathrm{d}}
\newcommand{\dq}{\, \mathrm{d} \mathbf{q}}
\newcommand{\dx}{\, \mathrm{d} \mathbf{x}}
\newcommand{\dxs}{\, \mathrm{d} \mathbf{x}\, \mathrm{d}\sigma}
\newcommand{\dt}{\, \mathrm{d}t}
\newcommand{\ds}{\, \mathrm{d}\sigma}
\newcommand{\dif}{\, \mathrm{d}}
\newcommand{\D}{\, \mathrm{d}}

\newcommand{\bk}{\mathbf{k}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\vu}{\mathbf{u}}

\newcommand{\bn}{\mathbf{n}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\sy}{\boldsymbol{\Psi}}
\newcommand{\py}{\boldsymbol{\Phi}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\vc}[1]{{\bf #1}}
\newcommand{\bs}[1]{{\boldsymbol{#1}}}
\newcommand{\mbf}[1]{{\mathbf{#1}}}
\newcommand{\mc}[1]{{\mathcal{#1}}}
\newcommand{\zh}{{\bs{\widehat z}}}

\newcommand{\Q}{\mathcal{Q}}

\newcommand{\dxt}{\,\mathrm{d}\mathbf{x}\, \mathrm{d}t}
\newcommand{\dqt}{\,\mathrm{d}\mathbf{q}\, \mathrm{d}t}
\newcommand{\dqxt}{\,\mathrm{d}\mathbf{q}\,\mathrm{d}\mathbf{x}\, \mathrm{d}t}

\newcommand{\expect}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}
\DeclareMathOperator*{\esssup}{ess\,sup}
\def\domain{\mathcal D}
\def\p{\partial}
\def\normal{\bf n}

\setlength\parindent{0pt}
\setlength{\parskip}{1em}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}


\usepackage{enumitem,amssymb}
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}%
\hspace{-2.5pt}}
\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}}
